Test Center Location Problem: A bi-objective Model and Algorithms

The optimal placement of healthcare facilities, including the placement of diagnostic test centers, plays a pivotal role in ensuring efficient and equitable access to healthcare services. However, the emergence of unique complexities in the context of a pandemic, exemplified by the COVID-19 crisis, has necessitated the development of customized solutions. This paper introduces a bi-objective integer linear programming model designed to achieve two key objectives: minimizing average travel time for individuals visiting testing centers and maximizing an equitable workload distribution among testing centers. To address this problem, we propose a customized local search algorithm based on the Voronoi diagram. Additionally, we employ an $\epsilon$-constraint approach, which leverages the Gurobi solver. We rigorously examine the effectiveness of the model and the algorithms through numerical experiments and demonstrate their capability to identify Pareto-optimal solutions. We show that while the Gurobi performs efficiently in small-size instances, our proposed algorithm outperforms it in large-size instances of the problem.

==> draft.tex <==
 

%The PSP has been widely studied to provide optimal scheduling solutions in the sectors like manufacturing, call centre, transportation, health-care since decades~\citep{baker1976workforce}. 

%The Personnel Scheduling problem (PSP) aims to determine an optimal workload distribution of staff that satisfies both the preferences of individuals and requirements of the organization [ref]. 

%In the literature, there exists different classifications of personnel scheduling problems.

%In general, depending on the time dependency of the scheduling structure, any scheduling problem can be labelled as either static or dynamic~\citep{ozder2020systematic}. 

%According to a popular classification, the personnel scheduling can also be categorized into (i) shift-scheduling, (ii) day-off scheduling, (iii) tour scheduling~\citep{baker1976workforce}. On the other hand, based on the methods applied to seek solutions of the personnel scheduling problem, it can be further classified as (i) linear programming problem or (ii) construction-based problem~\citep{bechtold1991comparative}. Further detailed review and other types of classification can be found in~\citep{van2013personnel,ozder2020systematic}. 

%Recently, in response to COVID-19 pandemic, personnel scheduling has gained more attention in different sectors such as service, retail, healthcare, and manufacturing; It helps to design strategies to avoid disruption work-flow in the organization during disease outbreak. 

%----------Literature review-------------------

%~\citep{moosavi2022staff} studied the problem of minimizing the cost associated with hiring part time staff members, over time of the staff members, and violation of time slot assigned for a particular task. 
%The problem was then further extended considering pandemic situation and introduced new objective function 
%that minimizes the number of unique staff members assigned to each room in the residential care and the number of distinct groups of residents served by each staff member. 


%Modelling this problem as a grouped weakly coupled dynamic program,~\citep{d2021optimal} proposed a prioritization scheme that schedules the patients for treatment based on their severity of health status, age group and applied this model to the National Health Service in England. %Schedule patients.

%It is noteworthy that in all of the aforementioned studies related to the personnel scheduling problem in a pandemic situation have not explicitly considered the important aspect in the optimization models: how the disease can be transmitted among the staffs in an organization? During the pandemic, since infection among the employees cause a great disruption in the workflow of the organizations, it becomes necessary to integrate disease transmission model into optimization model to gain better understanding on the complex interplay between the disease related factors and availability of resources in the organization.
%To this end, we develop a personnel scheduling model by explicitly integrating a probability based disease transmission model. \textbf{(MANSOOR or ANA Please Add more explanations when the introduction will be ready)}


